VFMF: World Modeling by Forecasting Vision Foundation Model Features

Forecasting from partial observations is central to world modeling. Many recent methods represent the world through images, and reduce forecasting to stochastic video generation. Although such methods excel at realism and visual fidelity, predicting pixels is computationally intensive and not directly useful in many applications, as it requires translating RGB into signals useful for decision making. An alternative approach uses features from vision foundation models (VFMs) as world representations, performing deterministic regression to predict future world states. These features can be directly translated into actionable signals such as semantic segmentation and depth, while remaining computationally efficient. However, deterministic regression averages over multiple plausible futures, undermining forecast accuracy by failing to capture uncertainty. To address this crucial limitation, we introduce a generative forecaster that performs autoregressive flow matching in VFM feature space. Our key insight is that generative modeling in this space requires encoding VFM features into a compact latent space suitable for diffusion. We show that this latent space preserves information more effectively than previously used PCA-based alternatives, both for forecasting and other applications, such as image generation. Our latent predictions can be easily decoded into multiple useful and interpretable output modalities: semantic segmentation, depth, surface normals, and even RGB. With matched architecture and compute, our method produces sharper and more accurate predictions than regression across all modalities. Our results suggest that stochastic conditional generation of VFM features offers a promising and scalable foundation for future world models.

==> convergence.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={\textbf{Training Steps}},
        ylabel={\textbf{FID}},
        width=0.5\textwidth,
        height=0.275\textwidth,
        grid=major,
        legend pos=north east,
        xmax=400000,
        ymin=0, % Start y-axis at 0
        enlarge y limits={upper, value=0.1}, % Add some padding at the top
        xtick={50000, 100000, 150000, 200000, 250000, 300000, 350000, 400000},
        xticklabels={50K, 100K, 150K, 200K, 250K, 300K, 350K, 400K},
        scaled x ticks=false, % <-- Prevents scientific notation
    ]
    % PCA data
    \addplot[mark=*, color=blue, thick] coordinates {
        (50000, 86.6396999)
        (100000, 47.66971024)
        (150000, 34.6757324)
        (200000, 28.56877841)
        (250000, 24.81495996)
        (300000, 22.18977025)
        (350000, 20.23456498)
        (400000, 18.49305575)
    };
    \addlegendentry{ReDi(PCA)}
    % VAE data
    \addplot[mark=square*, color=red, thick] coordinates {
        (50000, 63.08489057)
        (100000, 29.13829599)
        (150000, 21.94340577)
        (200000, 17.94953168)
        (250000, 15.56555068)
        (300000, 13.71012824)
        (350000, 12.54932724)
        (400000, 11.75866361)
    };
    \addlegendentry{ReDi(VAE)}
    \end{axis}
\end{tikzpicture}

==> sec/utils/definitions.tex <==
\newcommand{\csecond}[1]{\cellcolor{myyellow}#1}
\usepackage{mleftright}

\newcommand{\best}[1]{\colorbox{limegreen}{\textbf{#1}}}
\newcommand{\second}[1]{\colorbox{myyellow}{#1}}

% \renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\set}[1]{\mathcal{#1}}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\lossweight}{\lambda}
 
\newcommand{\geo}{\mathcal{S}}
\newcommand{\mesh}{\mathcal{M}}
\newcommand{\nerf}{\mathcal{N}}
\newcommand{\mlp}{f}
\newcommand{\backbone}{g}
\newcommand{\fullbackbone}{G}
\newcommand{\shadingnet}{s}
\newcommand{\weights}{\vec{\theta}}
\newcommand{\point}{\vec{x}}
\newcommand{\pointintersect}{\hat{\point}}
\newcommand{\gtpointintersect}{\bar{\point}}
% \newcommand{\normal}{\vec{n}}
% \newcommand{\normal}{\vec{N}}
\newcommand{\normal}{{N}}
\newcommand{\gtnormal}{\bar{\normal}}
\newcommand{\gtsdf}{\bar{\dist}}
% \newcommand{\image}{\mat{I}}
\newcommand{\pixel}{\vec{p}}
\newcommand{\pixelset}{\set{I}}
\newcommand{\mask}{\mat{M}}
\newcommand{\calibmatrix}{\mat{P}}
\newcommand{\albedoimg}{\mat{A}}
\newcommand{\front}{f}
\newcommand{\back}{b}
\newcommand{\encoding}{\gamma}
\newcommand{\dist}{d}
\newcommand{\albedo}{\vec{a}}
\newcommand{\gtalbedo}{\bar{\albedo}}
\newcommand{\cam}{\pi}
\newcommand{\signlabel}{l}
\newcommand{\patch}{p}
% \newcommand{\shading}{\vec{s}}
\newcommand{\shaded}{\vec{c}}
\newcommand{\ray}{\vec{r}}
\newcommand{\illum}{\vec{l}}
\newcommand{\illumnet}{l}
\newcommand{\rays}{\set{R}}
% \newcommand{\sigmoid}{\phi}
\newcommand{\sharpness}{k}
\newcommand{\origin}{\vec{o}}
% \newcommand{\sign}{\sigma}

% additional user-defined symbols
\newcommand{\misscite}{\textcolor{red}{[C]}}
\newcommand{\missref}{\textcolor{red}{[R]}}
\newcommand{\yslan}[1]{{\color{blue}(yslan: {#1})}} % yslan's comments
% for rebuttal mark
% \newcommand{\cm}[1]{{\color{black}{#1}}} % for rebuttal mark
% \newcommand*{\eg}{e.g.\@\xspace}
% \newcommand*{\ie}{i.e.\@\xspace}
%\newcommand{\ys}{\textcolor{magenta}}%magenta}}
% \usepackage[dvipsnames]{xcolor}
% \definecolor{magenta(process)}{rgb}{1.0, 0.0, 0.9}
% \newcommand{\ys}{\textcolor{magenta(process)}}%}}
\newcommand{\heading}[1]{\noindent\textbf{#1.}}

% \definecolor{jade}{rgb}{0.0, 0.66, 0.42}
% \newcommand{\shangchen}[1]{{\color{red}(SC: {#1})}} % shangchen's comments\textbf{}

% =========== Project Specific Definitions below
% \newcommand{\image}{\mat{I}}

% Paper Name
% \newcommand{\NICKNAME}{\textsc{Mono3Diff}} % temp "E"ncoder "3D" "G"an inv"E"rsion
% \newcommand{\NICKNAME}{\textsc{LN3Diff}} % temp "E"ncoder "3D" "G"an inv"E"rsion
% \newcommand{\NICKNAME}{\textsc{GaussianAnything}} % temp "E"ncoder "3D" "G"an inv"E"rsion
% \newcommand{\NICKNAME}{\textsc{STream3R}} % temp "E"ncoder "3D" "G"an inv"E"rsion
% \newcommand{\nickname}{\NICKNAME} % temp "E"ncoder "3D" "G"an inv"E"rsion
\newcommand{\SUPPLEMENTARY}{\textbf{Supplement}}

% 3D GAN related
% GAN
\newcommand{\rendererflag}{\mathbf{0}}
\newcommand{\decoderflag}{\mathbf{1}}

\newcommand{\rendererCode}{w_{\rendererflag}}
\newcommand{\decoderCode}{w_{\decoderflag}}

\newcommand{\generator}{G}
\newcommand{\rendererG}{\generator_{\rendererflag}}
\newcommand{\decoderG}{\generator_{\decoderflag}}

\newcommand{\rendererSpace}{\mathcal{W}+_{\rendererflag}}
\newcommand{\decoderSpace}{\mathcal{W}+_{\decoderflag}}

% encoder related
\newcommand{\encoder}{\mathrm{Encoder}}
\newcommand{\decoder}{\mathrm{Decoder}}
\newcommand{\decoderblk}{\mathrm{DecoderBlock}}
\newcommand{\head}{\mathrm{Head}}

% \newcommand{\pencode}{p_{\rm{Encoder}}}
% \newcommand{\pdecode}{p_{\rm{Decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\encoderGlobal}{\encoder_{\rendererflag}}
% \newcommand{\encoderLocal}{\encoder_{\decoderflag}}
% \newcommand{\encoderADA}{\encoder_\text{ADA}} % 


% space
\newcommand{\zspace}{\mathcal{Z}}
\newcommand{\wspace}{\mathcal{W}}
\newcommand{\wpspace}{\wspace+}


% 3D relevant
\newcommand{\surfaceset}{\set{P}_{\gO}}
\newcommand{\additionalset}{\set{P}_{\gF}}
\newcommand{\mlpGeo}{\phi_{g}}
\newcommand{\mlpFeature}{\phi_{f}}
\newcommand{\mlpTex}{\phi_{c}}
\newcommand{\view}{\bm{v}}

\newcommand{\campose}{\bm\xi}
\newcommand{\Refview}{\image_{\campose_{ref}}}
\newcommand{\Queryview}{\image_{\campose_{que}}}

% \newcommand{\depth}{\textbf{DEPTH}}
% \newcommand{\depth}{\bm{\Delta}} % in mcc
\newcommand{\depth}{{\Delta}} % in mcc

% \newcommand{\setsize}[1]{\left|{#1}\right|}
% \newcommand{\setsize}[1]{\mid{#1}\mid}
\newcommand{\setsize}[1]{|{#1}|}

\newcommand{\datasetsample}{\mathcal{X}}

% features
\newcommand{\feature}{\mathbf{F}} 
\newcommand{\featureLocal}{\feature_\text{L}} % ? check neuRay and mvsNeRF
% \newcommand{\featureGlobal}{\feature_{G}} % ? check neuRay and mvsNeRF

% Images
% \newcommand{\image}{\mat{I}}
% \newcommand{\image}{\mat{x}}
% \newcommand{\image}{x} % I stands for eye here
\newcommand{\image}{\bm{I}} % I stands for eye here
\newcommand{\rendering}{R} % I stands for eye here
\newcommand{\imageLowres}{\image_{lowres}}
\newcommand{\imageHighres}{\image_{highres}}
\newcommand{\imagePredicted}{\hat{\image}}
\newcommand{\imageEdit}{\image_{edit}}
\newcommand{\residual}{\Delta}

% from stylegan paper

\newcommand{\xx}{{\bf x}}
\newcommand{\yy}{{\bf y}}
\newcommand{\zz}{{\bf z}}
\newcommand{\ww}{{\bf w}}
\newcommand{\tildeww}{{\bf\tilde w}}
\newcommand{\barww}{{\bf\bar w}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\ZZ}{\mathcal{Z}}
\newcommand{\WW}{\mathcal{W}}
\newcommand{\MU}{\boldsymbol{\mu}}
\newcommand{\II}{\mathbf{I}}

\newcommand{\JJ}{{\bf J}}
\newcommand{\JJT}{{\bf J}^T}
\newcommand{\SSigma}{{\bf \Sigma}}
\newcommand{\real}{\mathbb{R}}
% \newcommand{\expectation}{\mathbb{E}}
\newcommand{\tyy}{\tilde {\bf y}}
\newcommand{\expectation}{\E}

% code
\newcommand{\zcode}{\zz}
\newcommand{\wcode}{\ww}
\newcommand{\wpcode}{{\wcode}+}
\newcommand{\wpcodeRenderer}{{\vw}+_{\rendererflag}}
\newcommand{\wpcodeDecoder}{{\vw}+_{\decoderflag}}

\newcommand{\RN}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}

% render

% \newcommand{\render}{\texttt{VolumeRender}}
\newcommand{\render}{\texttt{VR}}
\newcommand{\diffrender}{\texttt{R}}

% for 3dgs-like table
\definecolor{yellow}{rgb}{1, 1, 0.7}
\definecolor{orange}{rgb}{1, 0.85, 0.7}
\definecolor{tablered}{rgb}{1, 0.7, 0.7}
\definecolor{red}{rgb}{1, 0, 0}

\newcommand*{\Encoder}[1]{\textsc{Encoder}\mleft({#1}\mright)}
\newcommand*{\Decoder}[1]{\textsc{Decoder}\mleft({#1}\mright)}
\newcommand*{\Predictor}[1]{\textsc{Predictor}\mleft({#1}\mright)}
\newcommand*{\Attention}[1]{\textsc{Attention}\mleft({#1}\mright)}
\newcommand*{\CrossAttention}[2]{\textsc{CrossAttention}\mleft({#1}, {#2}\mright)}
\newcommand*{\Mlp}[1]{\textsc{MLP}\mleft({#1}\mright)}
\newcommand*{\LayerNorm}[1]{\textsc{LN}\mleft({#1}\mright)}

==> sec/utils/diffusion_commands.tex <==
% \newcommand{\projectpath}{https://github.com/CompVis/latent-diffusion}

\newcommand*{\approxident}{%
  \mathrel{\vcenter{\offinterlineskip
  \hbox{$\sim$}\vskip-.35ex\hbox{$\sim$}\vskip-.35ex\hbox{$\sim$}}}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\expec}{\mathbb{E}}
\newcommand{\prior}{\mathcal{N}(0,1)}


\newcommand{\xpixel}{x_\text{pixel}}
\newcommand{\xpixelrec}{\tilde{x}_\text{pixel}}
\newcommand{\hpixel}{H}
\newcommand{\wpixel}{W}
\newcommand{\cpixel}{3}
\newcommand{\xrec}{\tilde{x}}

\newcommand{\latent}{z_0}
\newcommand{\hlatent}{h}
\newcommand{\wlatent}{w}
\newcommand{\clatent}{c}

\newcommand{\zt}[1]{z_{#1}}
\newcommand{\enc}{E}
\newcommand{\ppixel}{p_\text{pixel}}
\newcommand{\pzt}[1]{p_{\zt{#1}}}
\newcommand{\qzt}[1]{q_{\zt{#1}}}
\newcommand{\q}{q}
% \newcommand{\R}{\mathbb{R}}

\newcommand{\LPIPS}{\text{LPIPS}}
% \newcommand{\KL}{\mathbb{KL}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\pmodel}[1]{p^{#1}_{\theta}}
\newcommand{\pchain}{p_{\theta}}
\newcommand{\qchain}{q}
\newcommand{\qmodel}[1]{q_{#1}}

\newcommand{\qenc}{q_{\phi}}
\newcommand{\pdec}{p_{\phi}}
\newcommand{\dec}{G_{\phi}}

\newcommand{\disc}{D_{\psi}}

\newcommand{\lrec}{L_{rec}}
\newcommand{\ladv}{L_{adv}}
\newcommand{\lreg}{L_{reg}}
\newcommand{\lcomp}{L_{cm}}
\newcommand{\lsimple}{L_{DM}}
\newcommand{\lsimpleldm}{\loss_{LDM}}
\newcommand{\lsimplediff}{\loss_\text{diff}}
\newcommand{\lsimplelcm}{L_{LDM}}

% \newcommand{\model}{\epsilon_\theta}
% \newcommand{\model}{\beps_\theta}
\newcommand{\model}{\beps_\Theta}
\newcommand{\modelforkl}{\beps_\xi}
\newcommand{\modelwithinp}{\model(\bz_t, t)}
\newcommand{\conditioner}{\tau_\theta}

\newcommand{\ldmencoder}{\mathcal{E}_\bphi}
\newcommand{\ldmdecoder}{\mathcal{D}_\bpsi}


\newcommand{\cond}{y}


% lsgm

% \newcommand{\KL}[2]{\text{KL}\!\left(#1 || #2\right)}
\newcommand{\ENTROPY}[1]{\text{H}\!\left(#1\right)}
\newcommand{\CE}[2]{\text{CE}(#1 || #2)}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bff}{{\mathbf{f}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bH}{{\text{\bf H}}}
\newcommand{\albar}{\bar{\alpha}}
\newcommand{\bebar}{\bar{\beta}}
\newcommand{\beps}{\boldsymbol{\epsilon}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bpsi}{{\boldsymbol{\psi}}}
\newcommand{\balpha}{{\boldsymbol{\alpha}}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\beye}{\mathbf{I}}
\newcommand{\betat}{\tilde{\beta}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\renewcommand{\det}{\Delta t}
\newcommand{\tdet}{t + \Delta t}
\newcommand{\tq}{{\tilde{q}}}
% \newcommand{\E}{{\mathbb{E}}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\U}{\mathcal{U}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\bmin}{\beta_{\text{min}}}
\newcommand{\bmax}{\beta_{\text{max}}}
\newcommand{\vmax}{\sigma^2_{\text{max}}}
\newcommand{\vmin}{\sigma^2_{\text{min}}}
% \newcommand{\vn}{\mathring{\sigma}^2}
\newcommand{\vsub}{\sigma_{\mathcal{N}_\textrm{Sub-VPSDE}}^2}
\newcommand{\sigo}{\sigma^2_0}
\newcommand{\sigt}{\sigma^2_t}
\newcommand{\vtil}{\tilde{\sigma}^2}


% \newcommand{\R}{\mathbb{R}}
\newcommand{\D}[1]{\dif #1}

% \newtheorem{theorem}{Theorem}

% \newcommand{\re}{\text{re}}
\newcommand{\un}{\text{un}}
\newcommand{\we}{\text{ll}}

==> sec/utils/macro.tex <==
\newcommand{\It}{\bm{I}_t}
\newcommand{\ft}{\bm{F}_t}
\newcommand{\fts}{\bm{F}_t'}
\newcommand{\stpre}{\bm{s}_{t-1}}
\newcommand{\stcur}{\bm{s}_{t}}
\newcommand{\zts}{\bm{z}_t'}
\newcommand{\pmself}{\hat{\bm X}_t^\text{local}}
\newcommand{\pmcross}{\hat{\bm X}_t^\text{global}}
\newcommand{\confself}{\bm C_t^\text{local}}
\newcommand{\confcross}{\bm C_t^\text{global}}
\newcommand{\headself}{\mathrm{Head}_\text{local}}
\newcommand{\headcross}{\mathrm{Head}_\text{global}}
\newcommand{\headpose}{\mathrm{Head}_\text{pose}}
\newcommand{\raymap}{\bm R}
\newcommand{\fr}{\bm{F}_r}
\newcommand{\frs}{\bm{F}_r'}
\newcommand{\headcolor}{\mathrm{Head}_\text{color}}
\newcommand{\pmselfset}{\mathcal{\hat{X}}^\text{local}}
\newcommand{\pmcrossset}{\mathcal{\hat{X}}^\text{global}}
\newcommand{\pose}{\hat{\bm P}_t}
\newcommand{\predrgb}{\hat{\bm I}_r}
\newcommand{\gtrgb}{{\bm I}_r}
\newcommand{\ourmethod}[0]{Ours}
\newcommand{\duster}[0]{DUSt3R}
\newcommand{\master}[0]{MASt3R}
\newcommand{\monster}[0]{MonST3R}
\newcommand{\spanner}[0]{Spann3R}

\newcommand{\gb}[1]{{\color{blue}GB: #1}}


==> sec/utils/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}
% \newcommand{\etal}{\textit{et al.}}
% Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}



% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}

\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\Vf{{\bm{F}}}
\def\Vz{{\bm{Z}}}

\def\Enc{{\bm{\phi}}}
\def\Dec{{\bm{\psi}}}


\renewcommand{\vec}[1]{\bm{#1}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{Encoder}}}
\newcommand{\pdecode}{p_{\rm{Decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
% $\newcommand{\Var}{\mathbb{Var}}$
% $\newcommand{\E}{\mathrm{E}}$
% $\newcommand{\Var}{\mathrm{Var}}$
% $\newcommand{\Cov}{\mathrm{Cov}}$ 
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Std}{\mathrm{Std}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


% \DeclarePairedDelimiter{\Norm}{\lVert}{\rVert}  %
% \DeclarePairedDelimiter{\Set}{\{}{\}}  %
\newcommand*{\SetDef}[2]{\{\, #1 \mid #2 \,\}}  %

\newcommand*{\Real}{\mathbb{R}}
\newcommand*{\Int}{\mathbb{Z}}
\newcommand*{\Natural}{\mathbb{N}}
\newcommand*{\Normal}{\mathcal{N}}

\newcommand*{\Tau}{\mathcal{T}}


==> sec/utils/used_macros.tex <==
\usepackage{amsmath,amsfonts,bm,mleftright}

\def\vv{{\bm{v}}}
\def\vf{{\bm{f}}}
\def\Vf{{\bm{F}}}
\def\Vz{{\bm{Z}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}
\def\Enc{{\bm{\phi}}}
\def\Dec{{\bm{\psi}}}

\renewcommand{\vec}[1]{\bm{#1}}

\newcommand*{\Encoder}[1]{\textsc{Encoder}\mleft({#1}\mright)}
\newcommand*{\Decoder}[1]{\textsc{Decoder}\mleft({#1}\mright)}

\newcommand{\E}{\mathbb{E}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\missref}{\textcolor{red}{[R]}}
\newcommand{\misscite}{\textcolor{red}{[C]}}


==> tables/city.tex <==
% --- LaTeX Table: Model Benchmark Results (from TSV, Filtered) ---
% This table requires the \usepackage{booktabs}, \usepackage{siunitx}, and \usepackage{multirow} packages.
% Swapped 'mean_ae' to be under 'Normals' category.
% Filtered to only show 'ConvNeXt L' entries for 'Ours'.

\begin{table*}[h!]
\centering
\caption{\textbf{Dense Forecasting on CityScapes}. Our method considerably outperforms DINO-Foresight.}
\label{tab:kubric_benchmarks_filtered}
\small % Use a smaller font to help the table fit
\sisetup{round-mode=places, round-precision=3} % Round all numbers to 3 decimal places
\begin{tabular}{
  l 
  S[table-format=2.3]
  S[table-format=2.3]
  S[table-format=2.3]
  S[table-format=1.3]
  S[table-format=2.3]
  S[table-format=1.3]
}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Segmentation}} & \multicolumn{2}{c}{\textbf{Depth}} & \multicolumn{2}{c}{\textbf{Normals}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & {mIoU ($\uparrow$)} & {MO\_mIoU ($\uparrow$)} & {d1 ($\uparrow$)} & {abs\_rel ($\downarrow$)} & {a3 ($\uparrow$)} & {mean\_ae ($\downarrow$)} \\
\midrule

\multicolumn{7}{l}{\textit{initial context length = 1, roll out 9 frames}} \\
\midrule
DINO-Foresight & 31.6723200 & 22.0003990 & 70.7711720 & 0.2347890 & 84.8175590 & 5.3349400 \\

 
  \method (Mean) & 34.0493720 & 30.9368400 & 75.6294700 & 0.1970750 & 88.1053930 & 4.6296790 \\
  \method (Best) & 31.7376110 & 28.5584100 & 78.4707180 & 0.1809680 & 89.3183440 & 4.4354600 \\
\midrule
\multicolumn{7}{l}{\textit{initial context length = 2, roll out 8 frames}} \\
\midrule
DINO-Foresight & 39.3517920 & 32.2585910 & 74.3362090 & 0.2074690 & 87.1377460 & 4.8624950 \\
 
  \method (Mean) & 41.6865750 & 38.9196080 & 77.8557770 & 0.1819600 & 90.8074190 & 4.1243270 \\
  \method (Best) & 39.5664780 & 36.7041590 & 80.2416230 & 0.1666010 & 91.3180690 & 4.0390130 \\
\midrule

\multicolumn{7}{l}{\textit{initial context length = 3, roll out 7 frames}} \\
\midrule
DINO-Foresight & 41.8855950 & 35.6074060 & 75.9108380 & 0.1914300 & 88.4167280 & 4.6049470 \\
 
  \method (Mean) & 44.3126650 & 41.6401900 & 79.6406490 & 0.1670230 & 91.6613220 & 3.9466050 \\
  \method (Best) & 42.4148920 & 39.6591710 & 81.5310970 & 0.1566890 & 92.2587050 & 3.8478270 \\
\midrule

\multicolumn{7}{l}{\textit{initial context length = 4, roll out 6 frames}} \\
\midrule
DINO-Foresight & 44.7466030 & 38.9247470 & 77.6553680 & 0.1768210 & 89.8656370 & 4.3098360 \\
 
  \method (Mean) & 46.2500520 & 43.6556030 & 80.5694300 & 0.1584540 & 92.4275580 & 3.7920350 \\
  \method (Best) & 44.4885630 & 41.8167650 & 82.4149170 & 0.1495890 & 92.9491730 & 3.7120730 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/city_kubric.tex <==
% --- LaTeX Table: Combined Benchmark Results (Highly Compressed, v4) ---
% This table requires the \usepackage{booktabs}, \usepackage{siunitx}, and \usepackage{multirow} packages.
% Modified for a single, narrow column. Parentheses removed from context header.

\begin{table}[ht!]
\centering
\caption{\textbf{Dense Future Forecasting Accuracy.} Our \textit{generative} \method considerably outperforms \textit{deterministic} DINO-Foresight on both CityScapes and Kubric, highlighting benefits of explicit modeling of uncertainty in future. \yslan{please textbf the best results, and explain the trend, with longer context and longer/smaller rollout, how the metrics change.}}
\label{tab:forecasting_narrow_compressed}
\footnotesize % Use a small font
\setlength{\tabcolsep}{2pt} % Further reduced column padding
\sisetup{
  round-mode=places,
  round-precision=2 % Rounding to 2 decimal places
}
\begin{tabular}{
  l 
  S[table-format=2.2] % Changed from 2.3
  S[table-format=2.2] % Changed from 2.3
  S[table-format=2.2] % Changed from 2.3
  S[table-format=1.2] % Changed from 1.3
  S[table-format=2.2] % Changed from 2.3
  S[table-format=1.2] % Changed from 1.3
}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Segmentation}} & \multicolumn{2}{c}{\textbf{Depth}} & \multicolumn{2}{c}{\textbf{Normals}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 % Abbreviated headers, arrows in ( )
 & {All ($\uparrow$)} & {Mov. ($\uparrow$)} & {d1 ($\uparrow$)} & {AbsRel ($\downarrow$)} & {a3 ($\uparrow$)} & {MeanAE ($\downarrow$)} \\
\midrule

% --- Context Length 1 ---
\multicolumn{7}{l}{\textit{Initial Context Length $|\mathcal{C}|$ = 1}} \\
\midrule
\multicolumn{7}{l}{\textbf{CityScapes} (\textit{roll out future 9 frames})} \\
\quad DINO-Foresight & 31.6723200 & 22.0003990 & 70.7711720 & 0.2347890 & 84.8175590 & 5.3349400 \\
\quad \method (Mean) & \textbf{34.05} & 30.9368400 & 75.6294700 & 0.1970750 & 88.1053930 & 4.6296790 \\
\quad \method (Best) & 31.7376110 & 28.5584100 & 78.4707180 & 0.1809680 & 89.3183440 & 4.4354600 \\
\midrule
\multicolumn{7}{l}{\textbf{Kubric} (\textit{roll out future 11 frames})} \\
\quad DINO-Foresight & 46.728558 & 5.106874 & 64.370214 & 0.24366 & 90.617921 & 2.937612 \\
\quad \method (Mean) & 48.289867 & 6.611382 & 68.326973 & 0.205459 & 93.29122 & 2.144349 \\
\quad \method (Best) & 70.553193 & 47.770578 & 88.803406 & 0.079166 & 93.451126 & 2.07245 \\
\midrule

% --- Context Length 2 ---
\multicolumn{7}{l}{\textit{Initial Context Length $|\mathcal{C}|$ = 2}} \\
\midrule
\multicolumn{7}{l}{\textbf{CityScapes} (\textit{roll out future 8 frames})} \\
\quad DINO-Foresight & 39.3517920 & 32.2585910 & 74.3362090 & 0.2074690 & 87.1377460 & 4.8624950 \\
\quad \method (Mean) & 41.6865750 & 38.9196080 & 77.8557770 & 0.1819600 & 90.8074190 & 4.1243270 \\
\quad \method (Best) & 39.5664780 & 36.7041590 & 80.2416230 & 0.1666010 & 91.3180690 & 4.0390130 \\
\midrule
\multicolumn{7}{l}{\textbf{Kubric} (\textit{roll out future 10 frames})} \\
\quad DINO-Foresight & 51.145584 & 14.394726 & 62.600888 & 0.239131 & 89.196849 & 3.361023 \\
\quad \method (Mean) & 55.893142 & 21.676942 & 68.868614 & 0.224827 & 92.311776 & 2.386842 \\
\quad \method (Best) & 64.840392 & 37.971548 & 78.057762 & 0.156597 & 91.659134 & 2.594156 \\
\midrule

% --- Context Length 3 ---
\multicolumn{7}{l}{\textit{Initial Context Length $|\mathcal{C}|$ = 3}} \\
\midrule
\multicolumn{7}{l}{\textbf{CityScapes} (\textit{roll out future 7 frames})} \\
\quad DINO-Foresight & 41.8855950 & 35.6074060 & 75.9108380 & 0.1914300 & 88.4167280 & 4.6049470 \\
\quad \method (Mean) & 44.3126650 & 41.6401900 & 79.6406490 & 0.1670230 & 91.6613220 & 3.9466050 \\
\quad \method (Best) & 42.4148920 & 39.6591710 & 81.5310970 & 0.1566890 & 92.2587050 & 3.8478270 \\
\midrule
\multicolumn{7}{l}{\textbf{Kubric} (\textit{roll out future 9 frames})} \\
\quad DINO-Foresight & 54.278188 & 19.954559 & 66.758659 & 0.223816 & 89.425004 & 3.261334 \\
\quad \method (Mean) & 59.466175 & 27.78518 & 71.934597 & 0.20883 & 92.671788 & 2.261647 \\
\quad \method (Best) & 68.253569 & 43.737385 & 80.092049 & 0.141566 & 92.313614 & 2.400157 \\
\midrule

% --- Context Length 4 ---
\multicolumn{7}{l}{\textit{Initial Context Length $|\mathcal{C}|$ = 4}} \\
\midrule
\multicolumn{7}{l}{\textbf{CityScapes} (\textit{roll out future 6 frames})} \\
\quad DINO-Foresight & 44.7466030 & 38.9247470 & 77.6553680 & 0.1768210 & 89.8656370 & 4.3098360 \\
\quad \method (Mean) & 46.2500520 & 43.6556030 & 80.5694300 & 0.1584540 & 92.4275580 & 3.7920350 \\
\quad \method (Best) & 44.4885630 & 41.8167650 & 82.4149170 & 0.1495890 & 92.9491730 & 3.7120730 \\
\midrule
\multicolumn{7}{l}{\textbf{Kubric} (\textit{roll out future 8 frames})} \\
\quad DINO-Foresight & 57.618561 & 25.778604 & 69.308382 & 0.215344 & 89.823544 & 3.113956 \\
\quad \method (Mean) & 61.741413 & 31.857861 & 71.876375 & 0.205571 & 92.66125 & 2.247179 \\
\quad \method (Best) & 69.863841 & 46.561631 & 80.498367 & 0.137018 & 92.621902 & 2.314139 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/heads_bold.tex <==
% --- Your Table ---
\begin{table}[ht!]
    \centering
    \footnotesize % Use a small font
    \caption{\textbf{Dense decoding performance of  decoding heads}, evaluated on ground truth annotated futures. Under equal latent capacity, PCA exhibits severe degradation, while the VAE maintains high reconstruction quality, significantly higher than PCA.}
    \label{tab:heads}
    \setlength{\tabcolsep}{2pt} % Reduced column padding
    \sisetup{
      round-mode=places,
      round-precision=2 % Rounding to 2 decimal places
    }
    % --- Column definition updated (swapped last two formats) ---
    \begin{tabular}{
      l                    % Model (left aligned)
      S[table-format=2.2]    % Seg All (↑)
      S[table-format=2.2]    % Seg Mov. (↑)
      S[table-format=2.2]    % Depth d1 (↑)
      S[table-format=1.2]    % Depth AbsRel (↓)
      S[table-format=2.2]    % Normals a3 (↑) - WAS 1.2
      S[table-format=1.2]    % Normals MeanAE (↓) - WAS 2.2
    }
    \toprule
    % --- Row 1 Headers (Updated) ---
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Segmentation}} & \multicolumn{2}{c}{\textbf{Depth}} & \multicolumn{2}{c}{\textbf{Normals}} \\
    % --- Cmidrules updated (column indices shifted) ---
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    % --- Row 2 Headers (Updated, \textbf removed) ---
     & {All ($\uparrow$)} & {Mov. ($\uparrow$)} & {d1 ($\uparrow$)} & {AbsRel ($\downarrow$)} & {a3 ($\uparrow$)} & {MeanAE ($\downarrow$)} \\
    \midrule
    % --- Section Header (Updated to 7 columns) ---
    \multicolumn{7}{l}{\textbf{Cityscapes}} \\
    % --- Data Rows (Last two columns swapped) ---
    \quad Direct DINO & {\textbf{68.42}} & 66.80571746826172 & {\textbf{87.18}} & {\textbf{0.11}} & 96.925926 & 2.938775 \\
    \quad PCA (1152) & 68.09736633300781 & {\textbf{67.28}} & 85.73092818260193 & 0.11500895023345947 & {\textbf{96.98}} & {\textbf{2.91}} \\
    \quad PCA (16) & 54.65583801269531 & 49.64780807495117 & 81.5988302230835 & 0.15756788849830627 & 94.76048278808594 & 3.4985973834991455 \\
    \quad VAE(16) & 65.64169311523438 & 64.31041717529297 & 84.75431203842163&  0.12315826117992401& 96.94222259521484 & 2.917991876602173\\
    \midrule
    % --- Section Header (Updated to 7 columns) ---
    \multicolumn{7}{l}{\textbf{Kubric}} \\
    % --- Data Rows (Last two columns swapped) ---
    \quad Direct DINO & {\textbf{99.54}} & {\textbf{99.16}} & 77.62729525566101 &  0.15639297664165497 &  {\textbf{99.62}} & 0.28796741366386414 \\
    \quad PCA (1152) & 99.49028778076172 & 99.0764389038086 &  77.51978039741516 & {\textbf{0.15}} & 99.61569213867188 & {\textbf{0.29}} \\
    \quad PCA (16) & 97.4259033203125 & 95.34408569335938 & 77.45527029037476& 0.15866990387439728 & 99.06644439697266& 0.4457050561904907 \\
    \quad VAE(16)  & 99.16780853271484 & 98.49254608154297 &  {\textbf{78.02}} &  0.15711060166358948& 99.55836486816406 &  0.302557110786438 \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/kubric.tex <==
% --- LaTeX Table: Model Benchmark Results (Corrected Headers) ---
% This table requires the \usepackage{booktabs}, \usepackage{siunitx}, and \usepackage{multirow} packages.
% Swapped 'mean_ae' to be under 'Normals' category.

\begin{table*}[h!]
\centering
\caption{\textbf{Dense Forecasting on Kubric}. Our method considerably outperforms DINO-Foresight.}
\label{tab:kubric_benchmarks_corrected}
\small % Use a smaller font to help the table fit
\sisetup{round-mode=places, round-precision=3} % Round all numbers to 3 decimal places
\begin{tabular}{
  l 
  S[table-format=2.3]
  S[table-format=2.3]
  S[table-format=2.3]
  S[table-format=1.3]
  S[table-format=2.3] % a3
  S[table-format=1.3] % mean_ae
}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Segmentation}} & \multicolumn{2}{c}{\textbf{Depth}} & \multicolumn{2}{c}{\textbf{Normals}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
 & {mIoU ($\uparrow$)} & {MO\_mIoU ($\uparrow$)} & {d1 ($\uparrow$)} & {abs\_rel ($\downarrow$)} & {a3 ($\uparrow$)} & {mean\_ae ($\downarrow$)} \\
\midrule

% --- Context Length 1 ---
\multicolumn{7}{l}{\textit{Initial context length = 1, roll out 11 frames}} \\
\midrule
DINO-Foresight & 46.728558 & 5.106874 & 64.370214 & 0.24366 & 90.617921 & 2.937612 \\
 
 \method (Mean) & 48.289867 & 6.611382 & 68.326973 & 0.205459 & 93.29122 & 2.144349 \\
 \method (Best) & 70.553193 & 47.770578 & 88.803406 & 0.079166 & 93.451126 & 2.07245 \\
\midrule

% --- Context Length 2 ---
\multicolumn{7}{l}{\textit{Initial context length = 2, roll out 10 frames}} \\
\midrule
DINO-Foresight & 51.145584 & 14.394726 & 62.600888 & 0.239131 & 89.196849 & 3.361023 \\
 
 \method (Mean) & 55.893142 & 21.676942 & 68.868614 & 0.224827 & 92.311776 & 2.386842 \\
 \method (Best) & 64.840392 & 37.971548 & 78.057762 & 0.156597 & 91.659134 & 2.594156 \\
\midrule

% --- Context Length 3 ---
\multicolumn{7}{l}{\textit{Initial context length = 3, roll out 9 frames}} \\
\midrule
DINO-Foresight & 54.278188 & 19.954559 & 66.758659 & 0.223816 & 89.425004 & 3.261334 \\
 
 \method (Mean) & 59.466175 & 27.78518 & 71.934597 & 0.20883 & 92.671788 & 2.261647 \\
 \method (Best) & 68.253569 & 43.737385 & 80.092049 & 0.141566 & 92.313614 & 2.400157 \\
\midrule

% --- Context Length 4 ---
\multicolumn{7}{l}{\textit{Initial context length = 4, roll out 8 frames}} \\
\midrule
DINO-Foresight & 57.618561 & 25.778604 & 69.308382 & 0.215344 & 89.823544 & 3.113956 \\
 
 \method (Mean) & 61.741413 & 31.857861 & 71.876375 & 0.205571 & 92.66125 & 2.247179 \\
 \method (Best) & 69.863841 & 46.561631 & 80.498367 & 0.137018 & 92.621902 & 2.314139 \\
\bottomrule
\end{tabular}
\end{table*}

% --- End of Table ---

==> tables/vit.tex <==
\begin{table}[h]
\centering
\caption{
    Hyperparameters for Symmetric ViT (Transformer) Models.
    Common parameters:
    \texttt{dinov2\_variant: "vitb14\_reg"},
    \texttt{feature\_stats: ".../dino.npz"},
    \texttt{intermediate\_layers: [2, 5, 8, 11]},
    \texttt{patch\_size: 14},
    \texttt{input\_dim: 3072},
    \texttt{latent\_channels: 16},
    \texttt{dropout: 0.1},
    \texttt{shape: [16, 16]},
    \texttt{use\_qk\_norm: true},
    \texttt{beta: 0},
    \texttt{abs\_pos\_enc: true}.
}
\label{tab:vit_hyperparams}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Hyperparameter} & \textbf{Base} (\texttt{symmetric\_vit\_base}) & \textbf{Large} (\texttt{symmetric\_vit\_large}) \\
\midrule
Encoder Layers        & 12   & 24   \\
Decoder Layers        & 12   & 24   \\
Heads                 & 12   & 16   \\
Hidden Dim            & 768  & 1024 \\
MLP Dim               & 3072 & 4096 \\
Num. Registers        & 4  & 4    \\
\bottomrule
\end{tabular}
\end{table}
